Pre-trained Model Guided Fine-Tuning for Zero-Shot Adversarial Robustness

Large-scale pre-trained vision-language models like CLIP have demonstrated impressive performance across various tasks, and exhibit remarkable zero-shot generalization capability, while they are also vulnerable to imperceptible adversarial examples. Existing works typically employ adversarial training (fine-tuning) as a defense method against adversarial examples. However, direct application to the CLIP model may result in overfitting, compromising the model's capacity for generalization. In this paper, we propose Pre-trained Model Guided Adversarial Fine-Tuning (PMG-AFT) method, which leverages supervision from the original pre-trained model by carefully designing an auxiliary branch, to enhance the model's zero-shot adversarial robustness. Specifically, PMG-AFT minimizes the distance between the features of adversarial examples in the target model and those in the pre-trained model, aiming to preserve the generalization features already captured by the pre-trained model. Extensive Experiments on 15 zero-shot datasets demonstrate that PMG-AFT significantly outperforms the state-of-the-art method, improving the top-1 robust accuracy by an average of 4.99%. Furthermore, our approach consistently improves clean accuracy by an average of 8.72%. Our code is available at https://github.com/serendipity1122/Pre-trained-Model-Guided-Fine-Tuning-for-Zero-Shot-Adversarial-Robustness.

==> experiment/cifar_clean.tex <==
\begin{table*}[htbp]
\centering
\caption{Zero-shot clean accuracies. 
We fine-tune the model on CIFAR100 \cite{krizhevsky2009learning} and evaluate six methods (rows) on 16 datasets (columns), presenting the accuracy for each dataset as well as the average accuracy.
After fine-tuning or adversarial fine-tuning on CIFAR100 \cite{krizhevsky2009learning}, the zero-shot accuracy of the CLIP model on clean images generally decreases.}
\label{tab:cifar-clean}
\begin{adjustbox}{width=\textwidth,keepaspectratio}
\begin{tabular}{lcccccccccccccccccc}
\toprule
% & \multicolumn{16}{c}{\textbf{Datasets}} \\ % 合并中间的列，并在合并的列上添加标题 "Datasets"
% \cmidrule(lr){2-17} % 这个命令将会在从第二列到第十三列的上方画一条线，'lr'是为了减少线的长度
Method    & \scriptsize\rotatebox{90}{CIFAR10 (\%)} & \scriptsize\rotatebox{90}{CIFAR100 (\%)} & \scriptsize\rotatebox{90}{STL10 (\%)} & \scriptsize\rotatebox{90}{SUN397 (\%)} & \scriptsize\rotatebox{90}{Food101 (\%)} & \scriptsize\rotatebox{90}{Oxfordpet (\%)} & \scriptsize\rotatebox{90}{Flowers102 (\%)} & \scriptsize\rotatebox{90}{DTD (\%)}   & \scriptsize\rotatebox{90}{EuroSAT (\%)} & \scriptsize\rotatebox{90}{Fgvc\_Aircraft (\%)} & \scriptsize\rotatebox{90}{TinyImageNet (\%)} & \scriptsize\rotatebox{90}{ImageNet (\%)} & \scriptsize\rotatebox{90}{Caltech101 (\%)} & \scriptsize\rotatebox{90}{Caltech256 (\%)} & \scriptsize\rotatebox{90}{StanfordCars (\%)} & \scriptsize\rotatebox{90}{PCAM (\%)}  & Average (\%) & Time (s) \\ 
\midrule
CLIP          & 88.28          & 63.47          & 97.65          & 55.06          & 76.79          & 85.93         & 48.43          & 43.75          & 45.31          & 8.20           & 59.18          & 62.65          & 32.22          & 86.13          & 54.10          & 52.67          & 59.98 & 0 \\ \hline
FT-Standard   & 91.21          & 77.73          & 97.46          & 55.02          & 68.82          & 84.37         & 38.86          & 43.75          & 37.82          & 13.28          & 49.21          & 54.49          & 28.71          & 78.12          & 49.41          & 46.15          & 57.15 &101 \\
FT-TeCoA \cite{mao2022understanding}      & 85.93   & 69.53    & 95.31 & 55.04  & 69.60   & 85.54     & 37.89      & 42.57 & 32.16   & 8.59           & 50.78        & 56.60         & 28.12        & 80.99 & 51.56 & 45.14 & 55.95 &253 \\
PMG-AFT (ours)         & 80.86   & 60.15    & 95.31 & 57.12  & 72.81   & 83.20     & 41.40      & 42.58 & 31.32   & 8.20           & 46.48        & 60.15         & 30.85        & 84.04 & 54.49 & 58.03 & 56.68 &377 \\ \hline
VPT-TeCoA \cite{mao2022understanding}     & 78.71   & 57.03    & 83.91 & 30.92  & 24.76   & 37.89     & 11.97      & 21.09 & 12.57   & 1.56           & 38.08        & 25.00         & 26.36        & 48.11 & 11.52 & 56.30 & 35.36 &350\\
VPT-PMG-AFT (ours)       & 83.59   & 61.13    & 85.54 & 38.55  & 39.53   & 49.60     & 16.66      & 33.59 & 13.13   & 14.06          & 40.23        & 33.51         & 24.60        & 61.65 & 23.63 & 59.73 & 42.42 &670\\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-5mm}
\end{table*}

==> experiment/cifar_robust.tex <==
\begin{table*}[htbp]
\centering
\caption{Adversarial zero-shot robust accuracies under PGD-10 \cite{madry2017towards} attack. We fine-tune the model on CIFAR100 \cite{krizhevsky2009learning} and evaluate six methods (rows) on 16 datasets (columns), presenting the accuracy for each dataset as well as the average accuracy, with the best results shown in bold. 
Here, CLIP represents the pre-trained CLIP model, while FT-standard refers to the model fine-tuned on clean datasets.}
\label{tab:cifar-robust}
\begin{adjustbox}{width=\textwidth,keepaspectratio}
\begin{tabular}{lcccccccccccccccccc}
\toprule
% & \multicolumn{16}{c}{\textbf{Datasets}} \\ % 合并中间的列，并在合并的列上添加标题 "Datasets"
% \cmidrule(lr){2-17} % 这个命令将会在从第二列到第十三列的上方画一条线，'lr'是为了减少线的长度
Method    & \scriptsize\rotatebox{90}{CIFAR10 (\%)} & \scriptsize\rotatebox{90}{CIFAR100 (\%)} & \scriptsize\rotatebox{90}{STL10 (\%)} & \scriptsize\rotatebox{90}{SUN397 (\%)} & \scriptsize\rotatebox{90}{Food101 (\%)} & \scriptsize\rotatebox{90}{Oxfordpet (\%)} & \scriptsize\rotatebox{90}{Flowers102 (\%)} & \scriptsize\rotatebox{90}{DTD (\%)}   & \scriptsize\rotatebox{90}{EuroSAT (\%)} & \scriptsize\rotatebox{90}{Fgvc\_Aircraft (\%)} & \scriptsize\rotatebox{90}{TinyImageNet (\%)} & \scriptsize\rotatebox{90}{ImageNet (\%)} & \scriptsize\rotatebox{90}{Caltech101 (\%)} & \scriptsize\rotatebox{90}{Caltech256 (\%)} & \scriptsize\rotatebox{90}{StanfordCars (\%)} & \scriptsize\rotatebox{90}{PCAM (\%)}  & Average (\%) & Time (s) \\ 
\midrule
CLIP           & 45.70          & 19.53          & 68.35          & 9.62           & 3.12          & 9.76           & 3.51           & 21.87          & 3.64           & 0.39           & 0.39          & 6.44           & 15.62          & 23.11          & 2.73          & 50.27          & 17.75    &0 \\ \hline
FT-Standard    & 27.34          & 15.43          & 57.03          & 10.01          & 3.20          & 5.85           & 4.10           & 17.18          & 0.65           & 0.00           & 0.00          & 6.83           & 16.60          & 22.46          & 2.53          & 35.65          & 14.05  &101 \\
FT-TeCoA \cite{mao2022understanding}       & 58.20          & \textbf{39.25} & 66.40          & 13.79          & 4.60          & 11.71          & 9.76           & 21.09          & 11.13          & 0.39           & 1.17          & 8.90           & 18.94          & 29.10          & 5.26          & 41.96          & 21.35  &253 \\
PMG-AFT (ours)         & \textbf{64.06} & 36.33          & \textbf{70.12} & \textbf{17.93} & \textbf{7.50} & \textbf{22.66} & \textbf{10.55} & \textbf{30.86} & \textbf{22.92} & \textbf{1.17}  & \textbf{2.73} & \textbf{10.51} & \textbf{21.09} & \textbf{34.83} & \textbf{5.46} & \textbf{58.37} & \textbf{26.06}  & 377\\ \hline
VP-TeCoA  \cite{mao2022understanding}     & 54.68          & 37.89          & 47.26          & 6.15           & 1.95          & 5.46           & 10.15          & 1.56           & 0.21           & 0.00           & 2.14          & 3.82           & 13.27          & 15.43          & 0.97          & 52.12          & 15.81  & 350\\
VPT-PMG-AFT (ours)         & \textbf{61.52} & \textbf{41.01} & \textbf{53.90}  & \textbf{8.24}  & \textbf{3.51} & \textbf{7.81}  & \textbf{10.41} & \textbf{2.34}  & \textbf{0.85}  & \textbf{1.17}  & \textbf{2.53} & \textbf{5.35}  & \textbf{13.47}          & \textbf{28.90 }         & \textbf{3.32}         & \textbf{55.16}          & \textbf{18.71}  &670\\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-3mm}
\end{table*}

==> experiment/layer_detail_clean.tex <==
\begin{table*}[hbpt]
\centering
\caption{Zero-shot clean accuracies. We fine-tune the model on TinyImageNet \cite{deng2009imagenet} by our method under the selection of different feature layers and distance metric. We evaluate on 16 datasets (columns), presenting the accuracy for each dataset as well as the average accuracy, with the best average result shown in bold.}
\label{tab:layer_clean}
\begin{adjustbox}{width=\textwidth,keepaspectratio}
\begin{tabular}{lccccccccccccccccc}
\toprule
% & \multicolumn{16}{c}{\textbf{Datasets}} \\ % 合并中间的列，并在合并的列上添加标题 "Datasets"
% \cmidrule(lr){2-17} % 这个命令将会在从第二列到第十三列的上方画一条线，'lr'是为了减少线的长度
Method    & \scriptsize\rotatebox{90}{CIFAR10 (\%)} & \scriptsize\rotatebox{90}{CIFAR100 (\%)} & \scriptsize\rotatebox{90}{STL10 (\%)} & \scriptsize\rotatebox{90}{SUN397 (\%)} & \scriptsize\rotatebox{90}{Food101 (\%)} & \scriptsize\rotatebox{90}{Oxfordpet (\%)} & \scriptsize\rotatebox{90}{Flowers102 (\%)} & \scriptsize\rotatebox{90}{DTD (\%)}   & \scriptsize\rotatebox{90}{EuroSAT (\%)} & \scriptsize\rotatebox{90}{Fgvc\_Aircraft (\%)} & \scriptsize\rotatebox{90}{TinyImageNet (\%)} & \scriptsize\rotatebox{90}{ImageNet (\%)} & \scriptsize\rotatebox{90}{Caltech101 (\%)} & \scriptsize\rotatebox{90}{Caltech256 (\%)} & \scriptsize\rotatebox{90}{StanfordCars (\%)} & \scriptsize\rotatebox{90}{PCAM (\%)}  & Average (\%) \\ 
\midrule
Output + KL          & 83.98  & 58.39  & 92.97  & 56.41  & 66.40  & 84.76  & 42.96  & 41.02  & 35.28  & 6.25   & 46.87   & 56.75   & 30.46   & 82.94   & 48.24   & 48.24   &\textbf{55.71}     \\
Output + $L_2$    & 68.55 & 43.55 & 89.45 & 50.33 & 54.06 & 74.21 & 36.32 & 36.71 & 21.68 & 7.81  & 49.02 & 46.32 & 28.51 & 73.11 & 39.84 & 51.95 & 48.21  \\ 
Feature + $L_2$       & 59.18 & 31.83 & 86.52 & 33.73 & 31.40  & 42.18 & 21.09 & 17.96 & 15.90  & 17.57 & 56.05 & 33.59 & 25.19 & 59.44 & 22.26 & 59.31 & 38.32  \\
Feature + COS       & 80.66 & 48.63 & 93.55 & 55.52 & 67.10  & 68.35 & 39.58 & 35.93 & 36.29 & 16.79 & 42.38 & 54.18 & 24.41 & 81.90  & 49.21 & 53.24 & 52.98  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> experiment/layer_detail_robust.tex <==
\begin{table*}[htbp]
\centering
\caption{Adversarial zero-shot robust accuracies under PGD-10 \cite{madry2017towards} attack. We fine-tune the model on TinyImageNet \cite{deng2009imagenet} by our method under the selection of different feature layers and distance metric. We evaluate on 16 datasets (columns), presenting the accuracy for each dataset as well as the average accuracy, with the best results shown in bold.}
\label{tab:layer_robust}
\begin{adjustbox}{width=\textwidth,keepaspectratio}
\begin{tabular}{lccccccccccccccccc}
\toprule
% & \multicolumn{16}{c}{\textbf{Datasets}} \\ % 合并中间的列，并在合并的列上添加标题 "Datasets"
% \cmidrule(lr){2-17} % 这个命令将会在从第二列到第十三列的上方画一条线，'lr'是为了减少线的长度
Method    & \scriptsize\rotatebox{90}{CIFAR10 (\%)} & \scriptsize\rotatebox{90}{CIFAR100 (\%)} & \scriptsize\rotatebox{90}{STL10 (\%)} & \scriptsize\rotatebox{90}{SUN397 (\%)} & \scriptsize\rotatebox{90}{Food101 (\%)} & \scriptsize\rotatebox{90}{Oxfordpet (\%)} & \scriptsize\rotatebox{90}{Flowers102 (\%)} & \scriptsize\rotatebox{90}{DTD (\%)}   & \scriptsize\rotatebox{90}{EuroSAT (\%)} & \scriptsize\rotatebox{90}{Fgvc\_Aircraft (\%)} & \scriptsize\rotatebox{90}{TinyImageNet (\%)} & \scriptsize\rotatebox{90}{ImageNet (\%)} & \scriptsize\rotatebox{90}{Caltech101 (\%)} & \scriptsize\rotatebox{90}{Caltech256 (\%)} & \scriptsize\rotatebox{90}{StanfordCars (\%)} & \scriptsize\rotatebox{90}{PCAM (\%)}  & Average (\%) \\ 
\midrule
Output + KL          & \textbf{66.99} & \textbf{38.28} & \textbf{76.17} & \textbf{24.23} & \textbf{14.92}& \textbf{33.59}& \textbf{23.43}& \textbf{34.38} & \textbf{24.15}& \textbf{3.91} & 14.84& \textbf{17.26}& \textbf{24.02} & \textbf{45.05} & \textbf{14.64}& \textbf{57.64} &\textbf{31.95}     \\
Output + $L_2$    & 41.21 & 24.41 & 70.50  & 20.61 & 14.45 & 31.25 & 22.85 & 28.90  & 14.38 & 0.78 & 19.53 & 17.46 & 24.21 & 41.60  & 11.91 & 51.67 & 27.23  \\ 
Feature + $L_2$       & 40.62 & 21.09 & 70.50  & 11.61 & 11.71 & 20.70  & 8.33  & 8.59  & 10.44 & 0.39 & 28.12 & 14.33 & 17.96 & 37.95 & 9.57  & 54.50  & 22.90  \\
Feature + COS       & 53.32 & 28.12 & 67.77 & 13.33 & 10.23 & 29.68 & 14.58 & 12.50  & 10.01 & 1.17 & 10.15 & 14.14 & 16.40  & 43.88 & 13.47 & 53.84 & 24.53  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> experiment/lossterm_detail_clean.tex <==
\begin{table*}[htbp]
\centering
\caption{Zero-shot clean accuracies. We fine-tune the model on TinyImageNet \cite{deng2009imagenet} by FT-TeCoA and our method with different loss function term coefficients and combinations. We evaluate on 16 datasets (columns), presenting the accuracy for each dataset as well as the average accuracy.
$\alpha$ and $\beta$ represent two hyper-parameters in the loss function $L=L_{robust}+\alpha L_{general}+\beta L_{clean}$.}
\label{tab:lossterm_detail_clean}
\begin{adjustbox}{width=\textwidth,keepaspectratio}
\begin{tabular}{lccccccccccccccccc}
\toprule
% & \multicolumn{16}{c}{\textbf{Datasets}} \\ % 合并中间的列，并在合并的列上添加标题 "Datasets"
% \cmidrule(lr){2-17} % 这个命令将会在从第二列到第十三列的上方画一条线，'lr'是为了减少线的长度
Method    & \scriptsize\rotatebox{90}{CIFAR10 (\%)} & \scriptsize\rotatebox{90}{CIFAR100 (\%)} & \scriptsize\rotatebox{90}{STL10 (\%)} & \scriptsize\rotatebox{90}{SUN397 (\%)} & \scriptsize\rotatebox{90}{Food101 (\%)} & \scriptsize\rotatebox{90}{Oxfordpet (\%)} & \scriptsize\rotatebox{90}{Flowers102 (\%)} & \scriptsize\rotatebox{90}{DTD (\%)}   & \scriptsize\rotatebox{90}{EuroSAT (\%)} & \scriptsize\rotatebox{90}{Fgvc\_Aircraft (\%)} & \scriptsize\rotatebox{90}{TinyImageNet (\%)} & \scriptsize\rotatebox{90}{ImageNet (\%)} & \scriptsize\rotatebox{90}{Caltech101 (\%)} & \scriptsize\rotatebox{90}{Caltech256 (\%)} & \scriptsize\rotatebox{90}{StanfordCars (\%)} & \scriptsize\rotatebox{90}{PCAM (\%)}  & Average (\%) \\ 
\midrule
FT-TeCoA \cite{mao2022understanding} ($\alpha=0,\beta=0$)          & 66.79 & 41.01 & 89.25 & 47.01 & 52.81 & 70.31 & 36.13 & 35.94 & 18.88 & 7.81 & 48.83 & 43.67 & 28.32 & 72.98 & 37.89 & 54.29 & 46.99     \\ \hline
PMG-AFT ($\alpha=1,\beta=0$) (ours)    & 86.52 & 65.43 & 95.89 & 57.81 & 71.95 & 83.20  & 44.14 & 42.18 & 46.41 & 9.37 & 61.13 & 60.62 & 24.21 & 80.07 & 43.94 & 59.61 & 58.28  \\ 
PMG-AFT ($\alpha=1,\beta=1$) (ours)       & 83.98 & 58.39 & 92.97 & 56.41 & 66.40  & 84.76 & 42.96 & 41.02 & 35.28 & 6.25 & 46.87 & 56.75 & 30.46 & 82.94 & 48.24 & 57.81 & 55.71  \\
PMG-AFT ($\alpha=2,\beta=1$) (ours)         & 87.30  & 59.76 & 94.33 & 57.58 & 71.09 & 84.37 & 43.75 & 40.62 & 51.56 & 7.42 & 35.54 & 58.94 & 31.44 & 83.46 & 51.95 & 56.19 & 57.20   \\ 
PMG-AFT ($\alpha=1,\beta=2$) (ours)     & 80.66 & 53.51 & 91.99 & 55.36 & 64.92 & 83.98 & 41.79 & 39.84 & 31.77 & 5.46 & 47.26 & 55.46 & 29.88 & 81.51 & 46.48 & 57.31 & 54.19   \\
PMG-AFT ($\alpha=0.5,\beta=1$) (ours)         & 77.93 & 51.56 & 91.40  & 53.92 & 63.51 & 82.81 & 42.18 & 38.67 & 28.97 & 6.25 & 50.39 & 54.10  & 29.29 & 80.40  & 45.89 & 56.75 & 53.37   \\
PMG-AFT ($\alpha=1,\beta=0.5$) (ours)         & 84.96 & 60.93 & 94.14 & 57.12 & 67.26 & 85.54 & 43.75 & 41.01 & 39.58 & 5.85 & 47.46 & 57.77 & 30.27 & 83.65 & 49.80  & 58.48 & 56.72   \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> experiment/lossterm_detail_robust.tex <==
\begin{table*}[htbp]
\centering
\caption{Adversarial zero-shot robust accuracies under PGD-10 \cite{madry2017towards} attack. We fine-tune the model on TinyImageNet \cite{deng2009imagenet} by FT-TeCoA and our method with different loss function term coefficients and combinations. We evaluate on 16 datasets (columns), presenting the accuracy for each dataset as well as the average accuracy, with the best average result shown in bold. $\alpha$ and $\beta$ represent two hyper-parameters in the loss function $L=L_{robust}+\alpha L_{general}+\beta L_{clean}$.}
\label{tab:lossterm_detail_robust}
\begin{adjustbox}{width=\textwidth,keepaspectratio}
\begin{tabular}{lccccccccccccccccc}
\toprule
% & \multicolumn{16}{c}{\textbf{Datasets}} \\ % 合并中间的列，并在合并的列上添加标题 "Datasets"
% \cmidrule(lr){2-17} % 这个命令将会在从第二列到第十三列的上方画一条线，'lr'是为了减少线的长度
Method    & \scriptsize\rotatebox{90}{CIFAR10 (\%)} & \scriptsize\rotatebox{90}{CIFAR100 (\%)} & \scriptsize\rotatebox{90}{STL10 (\%)} & \scriptsize\rotatebox{90}{SUN397 (\%)} & \scriptsize\rotatebox{90}{Food101 (\%)} & \scriptsize\rotatebox{90}{Oxfordpet (\%)} & \scriptsize\rotatebox{90}{Flowers102 (\%)} & \scriptsize\rotatebox{90}{DTD (\%)}   & \scriptsize\rotatebox{90}{EuroSAT (\%)} & \scriptsize\rotatebox{90}{Fgvc\_Aircraft (\%)} & \scriptsize\rotatebox{90}{TinyImageNet (\%)} & \scriptsize\rotatebox{90}{ImageNet (\%)} & \scriptsize\rotatebox{90}{Caltech101 (\%)} & \scriptsize\rotatebox{90}{Caltech256 (\%)} & \scriptsize\rotatebox{90}{StanfordCars (\%)} & \scriptsize\rotatebox{90}{PCAM (\%)}  & Average (\%) \\ 
\midrule
FT-TeCoA \cite{mao2022understanding} ($\alpha=0,\beta=0$)          & 40.82 & 24.41 & 70.70  & 19.21 & 14.45 & 28.13 & 23.05 & 28.13 & 12.57 & 3.13 & 19.33 & 16.48 & 24.02 & 40.56 & 12.69 & 53.68 & 26.96    \\ \hline
PMG-AFT ($\alpha=1,\beta=0$) (ours)    & 55.46 & 29.29 & 73.24 & 21.48 & 10.70  & 27.73 & 18.55 & 31.64 & 25.58 & 0.78 & 6.64  & 14.37 & 17.38 & 48.69 & 14.84 & 58.89 & 28.44  \\ 
PMG-AFT ($\alpha=1,\beta=1$) (ours)       & 66.99 & 38.28 & 76.17 & 24.23 & 14.92 & 33.59 & 23.43 & 34.38 & 24.15 & 1.56 & 14.84 & 17.26 & 24.21 & 45.05 & 14.64 & 57.64 & \textbf{31.95}  \\
PMG-AFT ($\alpha=2,\beta=1$) (ours)         & 69.72 & 34.76 & 74.02 & 21.57 & 10.07 & 29.29 & 17.96 & 33.20  & 30.79 & 0.78 & 6.25  & 14.06 & 22.07 & 39.51 & 11.13 & 56.02 & 29.45   \\ 
PMG-AFT ($\alpha=1,\beta=2$) (ours)     & 65.43 & 38.67 & 77.93 & 25.03 & 15.31 & 36.32 & 24.21 & 35.93 & 23.50  & 0.78 & 16.99 & 17.69 & 24.21 & 46.74 & 14.25 & 57.36 & 31.52   \\
PMG-AFT ($\alpha=0.5,\beta=1$) (ours)         & 58.00    & 34.76 & 75.00    & 24.41 & 16.01 & 34.76 & 24.80  & 33.20  & 19.85 & 0.39 & 18.75 & 18.12 & 23.43 & 46.68 & 15.82 & 56.64 & 31.28   \\
PMG-AFT ($\alpha=1,\beta=0.5$) (ours)         & 64.84 & 36.91 & 75.58 & 23.29 & 13.67 & 30.85 & 22.65 & 33.98 & 24.87 & 1.17 & 11.13 & 16.32 & 22.46 & 44.66 & 13.67 & 57.81 & 30.86   \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> experiment/strength_clean.tex <==
\begin{table*}[htbp]
\centering
\caption{Zero-shot clean accuracies. We fine-tune the model on TinyImageNet \cite{deng2009imagenet} with PGD-10 \cite{madry2017towards} of different perturbation bounds ($\varepsilon=1/255, 2/255$ and $4/255$) and evaluate on 16 datasets (columns), presenting the accuracy for each dataset as well as the average accuracy, with the best average result shown in bold.}
\label{tab:strength-clean}
\begin{adjustbox}{width=\textwidth,keepaspectratio}
\begin{tabular}{lccccccccccccccccc}
\toprule
% & \multicolumn{16}{c}{\textbf{Datasets}} \\ % 合并中间的列，并在合并的列上添加标题 "Datasets"
% \cmidrule(lr){2-17} % 这个命令将会在从第二列到第十三列的上方画一条线，'lr'是为了减少线的长度
Method    & \scriptsize\rotatebox{90}{CIFAR10 (\%)} & \scriptsize\rotatebox{90}{CIFAR100 (\%)} & \scriptsize\rotatebox{90}{STL10 (\%)} & \scriptsize\rotatebox{90}{SUN397 (\%)} & \scriptsize\rotatebox{90}{Food101 (\%)} & \scriptsize\rotatebox{90}{Oxfordpet (\%)} & \scriptsize\rotatebox{90}{Flowers102 (\%)} & \scriptsize\rotatebox{90}{DTD (\%)}   & \scriptsize\rotatebox{90}{EuroSAT (\%)} & \scriptsize\rotatebox{90}{Fgvc\_Aircraft (\%)} & \scriptsize\rotatebox{90}{TinyImageNet (\%)} & \scriptsize\rotatebox{90}{ImageNet (\%)} & \scriptsize\rotatebox{90}{Caltech101 (\%)} & \scriptsize\rotatebox{90}{Caltech256 (\%)} & \scriptsize\rotatebox{90}{StanfordCars (\%)} & \scriptsize\rotatebox{90}{PCAM (\%)}  & Average (\%) \\ 
\midrule
FT-TeCoA-1/255 \cite{mao2022understanding}          & 66.79  & 41.01  & 89.25  & 47.01  & 52.81  & 70.31  & 36.13  & 35.94  & 18.88  & 7.81   & 48.83   & 43.67   & 28.32   & 72.98   & 37.89   & 37.89   &46.99     \\
PMG-AFT-1/255(ours)    & 83.98  & 58.39  & 92.97  & 56.41  & 66.40  & 84.76  & 42.96  & 41.02  & 35.28  & 6.25   & 46.87   & 56.75   & 30.46   & 82.94   & 48.24   & 48.24   &\textbf{55.71}  \\ \hline
FT-TeCoA-2/255 \cite{mao2022understanding}       & 62.30  & 36.52 & 87.30  & 50.79 & 53.28 & 71.48 & 39.06 & 35.93 & 20.37 & 5.85 & 44.53 & 46.21 & 28.12 & 72.39 & 41.40  & 54.35 & 46.86  \\
PMG-AFT-2/255(ours)         & 78.12 & 54.29 & 91.01 & 56.94 & 65.15 & 85.54 & 41.01 & 37.89 & 31.96 & 4.29 & 35.15 & 54.60 & 29.49 & 79.29 & 46.09 & 54.68 & \textbf{52.84}   \\ \hline
FT-TeCoA-4/255  \cite{mao2022understanding}     & 62.50  & 38.86 & 89.45 & 57.33 & 63.59 & 80.46 & 42.96 & 37.50  & 29.36 & 3.51 & 40.82 & 53.94 & 28.12 & 76.95 & 42.07 & 49.88 & 49.83   \\
PMG-AFT-4/255(ours)         & 77.34 & 49.41 & 91.60  & 56.26 & 65.85 & 87.10  & 40.43 & 34.76 & 40.88 & 4.29 & 29.10  & 54.96 & 28.90  & 77.66 & 46.28 & 50.67 & \textbf{52.21}   \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> experiment/strength_robust.tex <==
\begin{table*}[htbp]
\centering
\caption{Adversarial zero-shot robust accuracies under PGD-10 \cite{madry2017towards} attack with different perturbation bounds ($\varepsilon=1/255, 2/255$ and $4/255$). We fine-tune the model on TinyImageNet \cite{deng2009imagenet} and evaluate on 16 datasets (columns), presenting the accuracy for each dataset as well as the average accuracy, with the best results shown in bold. We employ the same perturbation bound for both training and testing.}
\label{tab:strength-robust}
\begin{adjustbox}{width=\textwidth,keepaspectratio}
\begin{tabular}{lccccccccccccccccc}
\toprule
% & \multicolumn{16}{c}{\textbf{Datasets}} \\ % 合并中间的列，并在合并的列上添加标题 "Datasets"
% \cmidrule(lr){2-17} % 这个命令将会在从第二列到第十三列的上方画一条线，'lr'是为了减少线的长度
Method    & \scriptsize\rotatebox{90}{CIFAR10 (\%)} & \scriptsize\rotatebox{90}{CIFAR100 (\%)} & \scriptsize\rotatebox{90}{STL10 (\%)} & \scriptsize\rotatebox{90}{SUN397 (\%)} & \scriptsize\rotatebox{90}{Food101 (\%)} & \scriptsize\rotatebox{90}{Oxfordpet (\%)} & \scriptsize\rotatebox{90}{Flowers102 (\%)} & \scriptsize\rotatebox{90}{DTD (\%)}   & \scriptsize\rotatebox{90}{EuroSAT (\%)} & \scriptsize\rotatebox{90}{Fgvc\_Aircraft (\%)} & \scriptsize\rotatebox{90}{TinyImageNet (\%)} & \scriptsize\rotatebox{90}{ImageNet (\%)} & \scriptsize\rotatebox{90}{Caltech101 (\%)} & \scriptsize\rotatebox{90}{Caltech256 (\%)} & \scriptsize\rotatebox{90}{StanfordCars (\%)} & \scriptsize\rotatebox{90}{PCAM (\%)}  & Average (\%) \\ 
\midrule
FT-TeCoA-1/255 \cite{mao2022understanding}          & 40.82 & 24.41 & 70.70 & 19.21 & 14.45& 28.13& 23.05& 28.13 & 12.57& 3.13 & \textbf{19.33}& 16.48& 24.02 & 40.56 & 12.69& 53.68 &26.96     \\
PMG-AFT-1/255(ours)    & \textbf{66.99} & \textbf{38.28} & \textbf{76.17} & \textbf{24.23} & \textbf{14.92}& \textbf{33.59}& \textbf{23.43}& \textbf{34.38} & \textbf{24.15}& \textbf{3.91} & 14.84& \textbf{17.26}& \textbf{24.02} & \textbf{45.05} & \textbf{14.64}& \textbf{57.64} &\textbf{31.95}  \\ \hline
FT-TeCoA-2/255 \cite{mao2022understanding}       & 32.21          & 11.71          & 52.73          & 10.63          & 2.73          & 7.42           & \textbf{14.06} & 24.21          & 16.08          & \textbf{0.39} & \textbf{5.85} & 7.85           & 17.57          & 21.68          & 1.56          & 53.55          & 17.51  \\
PMG-AFT-2/255(ours)         & \textbf{63.28} & \textbf{26.56} & \textbf{66.79} & \textbf{13.83} & \textbf{3.18} & \textbf{7.64}  & 7.81           & \textbf{30.07} & \textbf{21.15} & 0.00             & 4.49          & \textbf{8.07}  & \textbf{18.16} & \textbf{27.66} & \textbf{1.95} & \textbf{54.79} & \textbf{22.21}   \\ \hline
FT-TeCoA-4/255  \cite{mao2022understanding}     & 29.29          & 9.18           & 46.28          & 4.63           & 0.39          & 0.00              & \textbf{0.78}  & 21.48          & 12.95          & 0.00             & 1.75          & 1.36           & 13.67          & 11.78          & 0.00             & 53.51          & 12.94   \\
PMG-AFT-4/255(ours)         & \textbf{63.28} & \textbf{21.87} & \textbf{59.96} & \textbf{7.17}  & \textbf{0.42} & \textbf{0.39}  & 0.58           & \textbf{26.56} & \textbf{20.11} & 0.00             & \textbf{1.95} & \textbf{1.36}  & \textbf{15.03} & \textbf{12.63} & \textbf{0.00}    & \textbf{53.57} & \textbf{17.80}   \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> sec/finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.
